Workload-Aware DRAM Error Prediction using Machine Learning

The aggressive scaling of technology may have helped to meet the growing demand for higher memory capacity and density, but has also made DRAM cells more prone to errors. Such a reality triggered a lot of interest in modeling DRAM behavior for either predicting the errors in advance or for adjusting DRAM circuit parameters to achieve a better trade-off between energy efficiency and reliability. Existing modeling efforts may have studied the impact of few operating parameters and temperature on DRAM reliability using custom FPGAs setups, however they neglected the combined effect of workload-specific features that can be systematically investigated only on a real system. In this paper, we present the results of our study on workload-dependent DRAM error behavior within a real server considering various operating parameters, such as the refresh rate, voltage and temperature. We show that the rate of single- and multi-bit errors may vary across workloads by 8x, indicating that program inherent features can affect DRAM reliability significantly. Based on this observation, we extract 249 features, such as the memory access rate, the rate of cache misses, the memory reuse time and data entropy, from various compute-intensive, caching and analytics benchmarks. We apply several supervised learning methods to construct the DRAM error behavior model for 72 server-grade DRAM chips using the memory operating parameters and extracted program inherent features. Our results show that, with an appropriate choice of program features and supervised learning method, the rate of single- and multi-bit errors can be predicted for a specific DRAM module with an average error of less than 10.5 %, as opposed to the 2.9x estimation error obtained for a conventional workload-unaware error model.

==> discussion.tex <==
\section{Future work}
\label{sec:future_work}

Previous studies have demonstrated several software-level optimizations that reduce the number of manifested DRAM errors~\cite{8046197}. Our model enables us to evaluate the effect of such optimizations on DRAM reliability without long running characterization campaigns that may take days, since the model predicts $WER$ and $P_{UE}$ for a specific workload under varying DRAM operating conditions for dozens of milliseconds.

In future work, we target to apply our model in heterogeneous-reliability memory frameworks where \trefp and \vdd are scaled only in DIMMs (an unreliable memory domain) used for allocation of user application data, but not the OS data~\cite{8613828}. The unreliable memory domain in such systems may not have any ECC protection mechanism to reduce the chip power. Thus, the proposed ML model enables to find a combination of compiler optimizations that minimizes the risk of single-bit errors when an application allocates data in the unreliable memory domain.

The ML model can be also applied in OS governors for automatic scaling of \trefp and \vdd in systems with enabled ECC to reduce the DRAM power without obtaining UEs that can disturb the system operation. Such governors may analyze program inherent features and the DRAM temperature for a workload at runtime, and predict \trefp and \vdd that do not trigger UEs for a specific workload.  

Overall, the presented model enables us for the first time to design and optimize software considering its effect on the error behavior of DRAM operating under varying operating parameters, identifying the optimal trade-off between DRAM reliability and energy efficiency. This work thus opens new avenues for research. 


